Machine Learning on Camera Images for Fast mmWave Beamforming

Perfect alignment in chosen beam sectors at both transmit- and receive-nodes is required for beamforming in mmWave bands. Current 802.11ad WiFi and emerging 5G cellular standards spend up to several milliseconds exploring different sector combinations to identify the beam pair with the highest SNR. In this paper, we propose a machine learning (ML) approach with two sequential convolutional neural networks (CNN) that uses out-of-band information, in the form of camera images, to (i) rapidly identify the locations of the transmitter and receiver nodes, and then (ii) return the optimal beam pair. We experimentally validate this intriguing concept for indoor settings using the NI 60GHz mmwave transceiver. Our results reveal that our ML approach reduces beamforming related exploration time by 93% under different ambient lighting conditions, with an error of less than 1% compared to the time-intensive deterministic method defined by the current standards.

==> Research_challenges.tex <==
\section{Research challenges}
This work is the first step towards implementing image driven beamforming in an experimental setup. Although the results are very promising, there are some challenges that need to be addressed. First, as any machine learning problem, the generality of the solution depends on the richness of the dataset. We have considered a reduced problem with 25 cases to verify our method. Without a shadow of a doubt, a generalized solution can be achieved by collecting data for more cases, i.e. different locations for the transmitter and receiver and the obstacle. Second, the antenna orientation plays a pivotal role in the best beam selection. One of the possible questions that can be addressed in the forthcoming works would be the extraction of orientation from the images and incorporating them in the prediction.   

